Automating Outlier Detection via Meta-Learning

Given an unsupervised outlier detection (OD) task on a new dataset, how can we automatically select a good outlier detection method and its hyperparameter(s) (collectively called a model)? Thus far, model selection for OD has been a "black art"; as any model evaluation is infeasible due to the lack of (i) hold-out data with labels, and (ii) a universal objective function. In this work, we develop the first principled data-driven approach to model selection for OD, called MetaOD, based on meta-learning. MetaOD capitalizes on the past performances of a large body of detection models on existing outlier detection benchmark datasets, and carries over this prior experience to automatically select an effective model to be employed on a new dataset without using any labels. To capture task similarity, we introduce specialized meta-features that quantify outlying characteristics of a dataset. Through comprehensive experiments, we show the effectiveness of MetaOD in selecting a detection model that significantly outperforms the most popular outlier detectors (e.g., LOF and iForest) as well as various state-of-the-art unsupervised meta-learners while being extremely fast. To foster reproducibility and further research on this new problem, we open-source our entire meta-learning system, benchmark environment, and testbed datasets.

==> TABLE/OD_models_short.tex <==
\begin{table}%[ht]
\centering
	\caption{Outlier Detection Models in \method} % title of Table
	\begin{tabular}{lccc } % centered columns (4 columns)
	    \toprule
		\textbf{Method} &
		\textbf{Parameter 1} & \textbf{Parameter 2}\\
		\midrule
        ABOD \shortcite{kriegel2008angle}                           & n\_neighbors   & N/A \\
		COF \shortcite{tang2002enhancing}                           & n\_neighbors   & N/A \\
        HBOS \shortcite{goldstein2012histogram}                     & n\_histograms  & tolerance  \\
        iForest \shortcite{liu2008isolation}	    	         	& n\_estimators  & max\_features \\
        kNN \shortcite{ramaswamy2000efficient}                      & n\_neighbors   & distance metric \\
		LODA \shortcite{pevny2016loda}                              & n\_bins        & n\_random\_cuts \\
        LOF \shortcite{breunig2000lof}                              & n\_neighbors   & distance metric \\
        OCSVM \shortcite{scholkopf2001estimating}                   & nu (train error tol)    & kernel  \\
		\bottomrule
	\end{tabular}
	\label{table:models_short} % is used to refer this table in the text
\end{table}

==> TABLE/run_time.tex <==
\begin{table}[!htp]
\scriptsize
\caption{\leman{this is not necessary - Fig 5 is enough to communicate that overhead is small. You can give in text average \% overhead. BTW how did you choose these 10 datasets? Looks arbitrary.}Runtime breakdown in seconds by \method (meta-feature generation and model selection with meta-features), and the actual training of the selected model. \method (meta-feature generation and model selection) incurs low overhead to the training of a selected model.}\label{table:runtime}
\begin{tabular}{l|rr|r | r}
\toprule
\textbf{Dataset} & \makecell{\textbf{Meta-Feature} \\ \textbf{Generation} (g)} & \makecell{\textbf{Model} \\ \textbf{Selection} (s)} & \makecell{\textbf{Model} \\ \textbf{Training} (t)} &  \makecell{\textbf{Overhead (\%)} \\ $(\text{g}+\text{s})/\text{t}$}\\
% $\frac{\text{g}+\text{s}}{\text{t}}$
\midrule
abalone       & 0.0367            & 0.2022           & 1.2326                & 19.39\% \\
gas           & 0.3264            & 0.2298           & 19.3698               & 2.87\%  \\
imgseg        & 0.0361            & 0.2133           & 0.6449                & 38.67\% \\
letter        & 0.0517            & 0.2415           & 5.8406                & 5.02\%  \\
magic         & 0.0713            & 0.2097           & 12.6051               & 2.23\%  \\
particle      & 0.5986            & 0.2004           & 28.6861               & 2.79\%  \\
skin          & 0.0492            & 0.2424           & 22.2726               & 1.31\%  \\
wave          & 0.0460            & 0.2180           & 2.8522                & 9.26\%  \\
wine          & 0.0529            & 0.2132           & 4.6906                & 5.67\%  \\
yearp         & 0.6090            & 0.2070           & 27.0062               & 3.02\%  \\
\bottomrule
\end{tabular}
\end{table}
